Verifying Programs with Logic and Extended Proof Rules: Deep Embedding v.s. Shallow Embedding

Many foundational program verification tools have been developed to build machine-checked program correctness proofs, a majority of which are based on Hoare logic. Their program logics, their assertion languages, and their underlying programming languages can be formalized by either a shallow embedding or a deep embedding. Tools like Iris and early versions of Verified Software Toolchain (VST) choose different shallow embeddings to formalize their program logics. But the pros and cons of these different embeddings were not yet well studied. Therefore, we want to study the impact of the program logic's embedding on logic's proof rules in this paper. This paper considers a set of useful extended proof rules, and four different logic embeddings: one deep embedding and three common shallow embeddings. We prove the validity of these extended rules under these embeddings and discuss their main challenges. Furthermore, we propose a method to lift existing shallowly embedded logics to deeply embedded ones to greatly simplify proofs of extended rules in specific proof systems. We evaluate our results on two existing verification tools. We lift the originally shallowly embedded VST to our deeply embedded VST to support extended rules, and we implement Iris-CF and deeply embedded Iris-Imp based on the Iris framework to evaluate our theory in real verification projects.

==> contents/7_sep.tex <==
\section{Discussion: Embeddings of Separation Logic and Procedure Calls}
\label{sec:hypo}

% done: embedding in separation logic
% how to realize frame rule in shallow embedding
% unchanged validity
% or use frame definition of validity

% in deep embedding need to put frame in leave proof rules

So far, we have discussed different embeddings of the conventional Hoare logic with control flows and their proofs for extended rules.
When reasoning about memory operations, it is useful to extend the Hoare logic to a separation logic \cite{reynolds02}.
A separation logic adds a logic connective, ``$*$'', separating conjunction, to the assertion language. The assertion $P * Q$ asserts two disjoint memory satisfying $P$ and $Q$ respectively.
Typically, a separation logic adds proof rules for memory related assignments (rules for load and store) and the \textsc{frame} rule to Hoare logic.
Also, when function call is involved in a programming language, separation logic allows verifiers to prove a Hoare triple about global memory while the callee function specification only states its local effects.
Additionally, O'Hearn \textit{et. al} \cite{o2004separation}
proposes hypothetical frame rule which makes related proofs more flexible.
% We also discuss procedure calls and the hypothetical frame rule in this section. 
Figure~\ref{fig:sep} below shows these rules. For paper demonstration, we only consider
\begin{itemize}
\item Simple load, $x = [y]$, where $x$ and $y$ are program variables, and this command loads the value from the location with address $y$ into variable $x$.
\item Simple store, $[x] = y$, where $x$ and $y$ are program variables, and this command stores the value of $y$ into the location with address $y$.
\item Simple procedure call, $\text{call} \ f()$, where procedure calls have no arguments or return value.
Function arguments and return values are written to specific locations to be transferred between the caller and the callee.
\end{itemize}

In addition, we assume that there is no memory load in an expression.
Every memory operation is performed as a load or store command.
This is similar to the Clight program in CompCert \cite{krebbers2014formal} and the C program in VST-Floyd \cite{VST-Floyd}.

In this section, we first consider program logics with load and store to discuss some basics of separation logic embeddings.
Then we introduce rules related to procedure calls above it and further discuss embeddings for the logic with procedure calls.

\subsection{Frame Rule and More Potential Shallow Embeddings}
\label{sec:frame}

Figure~\ref{fig:sep} extends our previous toy WhileCF language and logic with memory operations and related proof rules.
\textsc{hoare-load} and \textsc{hoare-store} are often admitted as primary rules, and we mainly discuss the \textsc{frame} rule in this paper.

\begin{figure}[h]
\paragraph{While-CF with Memory Operations}
$$
\begin{array}{rcl}
c \in \text{command} &:=& \cdots \ \mid \ x = [y] \ \mid \ [x] = y
\end{array}
$$
\paragraph{Separation Logic Proof Rules}
\begin{mathpar}
    \inferrule[hoare-load]{}{
        \vdash \triple{l \mapsto v \land \doublebrackets{y} = l}{\ \ x = [y] \ \ }{l \mapsto v \land  \doublebrackets{x} = v \land \doublebrackets{y} = l, [\bot, \bot]}}
    \and
    \inferrule[hoare-store]{}{
        \vdash \triple{l \mapsto v \land \doublebrackets{x} = l \land \doublebrackets{y} = u}{\ \ [x] = y \ \ }{l \mapsto u \land \doublebrackets{x} = l \land \doublebrackets{y} = u, [\bot, \bot]}}
    \and
    \inferrule[frame]{
        c \text{ does not modify program variables freely occurring in } $F$ \\\\
        \vdash \triple{P}{c}{Q, [Q_{\text{brk}}, Q_{\text{con}}]}
    }{
        \vdash \triple{P * F}{c}{Q * F, [Q_{\text{brk}} * F, Q_{\text{con}} * F]}
    }
\end{mathpar}
    \caption{Additional Proof Rules for Separation Logics}
    \label{fig:sep}
\end{figure}

The \textsc{frame} rule allows prover to remove unused separating conjuncts (assertions in separation logics) of memory from both pre-/post-conditions and prove the specification with remaining memories.
Gotsman \textit{et al.} \cite{gotsman2011precision} proved: if the operational semantics satisfies the frame property, then the \textsc{frame} rule will always generate valid conclusions from valid assumptions.
The following hypotheses state the frame property via a big-step semantics and via a small-step semantics.
We use $\sigma' \oplus \sigma$ to represent the disjoint union of two pieces of memory, $\sigma'$ and $\sigma$.

\begin{hypo}
\label{hyp:frame-big}
For any $c$, $\text{ek}$, $\sigma_1$, $\sigma'_2$ and $\sigma$,
\begin{itemize}
\item if $(c, \sigma_1 \oplus \sigma) \Uparrow$, then $(c, \sigma_1) \Uparrow$;
\item if $(c, \sigma_1 \oplus \sigma) \Downarrow (\text{ek}, \sigma'_2)$, then either $(c, \sigma_1) \Uparrow$ or
   $\sigma'_2 = \sigma_2 \oplus \sigma $ for some $\sigma_2$ and  $(c, \sigma_1) \Downarrow (\text{ek}, \sigma_2)$.
\end{itemize}
\end{hypo}

\begin{hypo} For any $c_1$, $c_2$, $\kappa_1$, $\kappa_2$, $\sigma_1$, $\sigma'_2$ and $\sigma$,
\begin{itemize}
\item if $(c_1, \kappa_1, \sigma_1 \oplus \sigma) \not\rightarrow_c$, then $(c_1, \kappa_1, \sigma_1) \not\rightarrow_c$;
\item if $(c_1, \kappa_1, \sigma_1 \oplus \sigma) \rightarrow_c (c_2, \kappa_2, \sigma'_2)$, then either $(c_1,\kappa_1,  \sigma_1)  \not\rightarrow_c$ or
   $\sigma'_2 = \sigma_2 \oplus \sigma $ for some $\sigma_2$ and  $(c_1, \kappa_1, \sigma_1) \rightarrow_c (c_2, \kappa_2, \sigma_2)$.
\end{itemize}
\end{hypo}

These two properties are true for most reasonable languages (including realistic languages like C). And Gotsman's conclusion holds for $\vDash_b$,  $\vDash_w$, and $\vDash_c$ (respectively stand for the validity definition under \textbf{\textit{b}}ig-step based embedding, \textbf{\textit{s}}mall-step based embedding, and \textbf{\textit{c}}ontinuation-based embedding).
For example, theorem~\ref{thm:frame-big} proves the \textsc{frame} rule in the big-step based embedding.

\begin{thm}
\label{thm:frame-big}
    The \textsc{frame} rule holds for the big-step based embedding defined in section~\ref{sec:embed-big}, if the hypothesis~\ref{hyp:frame-big} is true.
\end{thm}
\begin{proof}
To prove $\bigvalid \triple{P*F}{c}{Q*F, [R_\ekb*F, R_\ekc*F]}$, we need to show that for any $\sigma \vDash P*F$ (1) $\lnot\,(c, \sigma)\Uparrow$, and (2) $\text{for all } \ek, \sigma_2, \text{if }(c, \sigma) \Downarrow (\ek, \sigma_2)$, $\sigma_2$ satisfies corresponding post-conditions with the frame $F$ according to $\ek$.

According to the premise $\bigvalid \triple{P}{c}{Q, [R_\ekb, R_\ekc]}$, we know for any $\sigma_1 \vDash P$ (i) $\lnot\,(c, \sigma_1)\Uparrow$, and (ii) $\text{for all } \ek, \sigma_2, \text{if }(c, \sigma_1) \Downarrow (\ek, \sigma_2)$, $\sigma_2$ satisfies corresponding post-conditions without the frame $F$ according to $\ek$.

We can split $\sigma$, according to $\sigma \vDash P*F$, into $\sigma_1$ and $\sigma'$ satisfying
$$
\sigma = \sigma_1 \oplus \sigma' \quad\text{and}\quad \sigma_1 \vDash P \quad\text{and}\quad \sigma' \vDash F.
$$
By (i), we know $\lnot\,(c, \sigma_1)\Uparrow$. And by hypothesis~\ref{hyp:frame-big}, we have $\lnot\,(c, \sigma_1 \oplus \sigma')\Uparrow$ because otherwise we have a contradiction and we prove (1).

To prove (2), by hypothesis~\ref{hyp:frame-big}, for any $\ek, \sigma_2$ with $(c, \sigma_1 \oplus \sigma') \Downarrow (\ek, \sigma_2)$, we know that
\begin{itemize}
    \item either $(c, \sigma_1)\Uparrow$, which contradicts with the premise (i) and finishes the proof;
    \item or there exists $\sigma_2'$ with $\sigma_2 = \sigma_2' \oplus \sigma'$ and $(c, \sigma_1) \Downarrow (\ek, \sigma_2')$.
    By (ii), we know $\sigma_2'$ satisfies corresponding post-conditions without the frame $F$ according to $\ek$ (i.e., $\sigma_2' \vDash Q$, $\sigma_2' \vDash R_\ekb$, or $\sigma_2' \vDash R_\ekc$).
    Since $\sigma' \Vdash F$, we know $\sigma_2 = \sigma_2' \oplus \sigma'$ satisfies corresponding post-conditions with the frame $F$ according to $\ek$ (i.e., $\sigma_2 \vDash Q*F$, $\sigma_2 \vDash R_\ekb*F$, or $\sigma_2 \vDash R_\ekc*F$), which finishes the proof.
\end{itemize}
\end{proof}

Interestingly, a different style of shallow embeddings for separation logic \cite{torp2005semantics} are widely used and the \textsc{frame} rule will hold intrinsically.
The \textsc{frame} rule in this style is called the "baked-in frame rule" in some literatures.
It define the Hoare triple as: for any shallow embedding $\vDash_x$ among $\vDash_b$,  $\vDash_w$, and $\vDash_c$,
$$\vDash_{\text{sep}-x} \triple{P}{c}{Q, [R_\ekb, R_\ekc]} \ \text{iff. for any} \ F, \vDash_x \triple{P*F}{c}{Q*F, [R_\ekb * F, R_\ekc * F]}. $$
Taking continuation based shallow embedding for example, we can use another definition: $\vDash_{\text{sep}-c} \triple{P}{c}{Q, [R_\ekb, R_\ekc]}$ iff. for arbitrary continuation $\kappa$ and \textit{arbitrary frame $F$} (also a separation logic assertion),
$$
\text{if } \quad \begin{cases}
    \quad\guard{Q * F}{\cskip}{\kappa} \\
    \quad\guard{Q_\ekb * F}{\cbreak}{\kappa} \\
    \quad\guard{Q_\ekc * F}{\ccontinue}{\kappa} 
\end{cases}
\text{then } \quad \guard{P * F}{c}{\kappa}.
$$
This is the way how shallowly embedded VST defines its Hoare triples.
Under such embedding, we can easily verify the \textsc{frame} rule without using the frame property of small-step operational semantics.
The premise $\vDash_{\text{sep}-c}~\!\triple{P}{c}{Q, [R_\ekb, R_\ekc]}$ means that for arbitrary frame $F''$, $$\vDash_{c} \triple{P * F''}{c}{Q * F'', [R_\ekb * F'', R_\ekc * F'']}.$$
Let $F'' = F * F'$. Then we know $\vDash_{c} \triple{(P * F) * F'}{c}{(Q * F) * F', [(R_\ekb * F) * F', (R_\ekc * F) * F']}$ for any $F$ and $F'$, which exactly states the conclusion of \textsf{frame}:
$$\vDash_{\text{sep}-c} \triple{P*F}{c}{Q*F}.$$
Although such sep$-x$ embedding does not invalidate any primary rules or extended rules we have mentioned so far, it does make other proofs more complicated since we need to deals with this extra frame $F$.
In comparison, both embedding styles are feasible.
The original one makes proofs of other primary rules and extended rules relatively concise, while the sep$-x$ version makes the proof of the frame rule simple.

\subsection{Frame Rule and Deep Embeddings}
\label{sec:frame-dep}
In deeply embedded program logics, we can either choose to make \textsc{frame} a primary rule or treat it as an extended rule.

The former option means that the separation logic's soundness is based on the fact that \textsc{frame} preserves Hoare triple's validity.
This proof is very similar to the verification of \textsc{frame} in shallowly embedded logics.
When developing a deeply embedded logic based on a shallowly embedded logic (see section~\ref{sec:d2s}), one could directly reuse the proof of \textsc{frame} rule in the shallow embedding.
However, as discussed in previous sections, adding one more primary rule to the proof system may invalidate the other proofs because every case analysis and inductions on proof trees will have one more branch to prove.
In the case of \textsc{frame} rule, although extended rules we have discussed may not be invalidated by this extra case, such choice would cause more uncertainty when we want to add more extended rules where this extra case may be unprovable.
Keeping the proof system concise with only atomic rules, compositional rules, and the consequence rule will make the logic more extensible and thus we give up this design choice and prove frame rule as an extended rule.

Nevertheless, we are not yet able to prove it with our previous deeply embedded program logic by simple induction over the proof tree of $\triple{P}{c}{Q}$.
The induction steps of \textsc{hoare-load} and \textsc{hoare-store} are not provable.
We should allow these rules to be compatible with extra frames.
For example, we use \textsc{hoare-load-frame} to replace \textsc{hoare-load}.
\begin{mathpar}
    \inferrule[hoare-load-frame]{}{
        \vdash \triple{F * l \mapsto v \land \doublebrackets{y} = l}{\ \ x = [y] \ \ }{F * l \mapsto v \land  \doublebrackets{x} = v \land \doublebrackets{y} = l, [\bot, \bot]}}
\end{mathpar}
Then, we can easily prove the \textsc{frame} rule by induction over the proof tree.
Similarly, for a language with more commands, we only need to guarantee proof rules for memory related operations are compatible with extra frames.

\subsection{Hypothetical Frame Rule}
\label{sec:hypo-frame}

In this section, we further extend the language and logic in figure~\ref{fig:sep} with procedure calls.
Different from logics in previous sections, the judgement of the logic in figure~\ref{fig:sep-call} takes the form of $\Delta \vdash \triple{P}{c}{Q, [\vec{R}]}$.
Here, $\Delta$ is the function hypothesis (or type-context in VST), containing a list of Hoare triples $\triple{P_i}{k_i}{Q_i}$ specifying the pre/post-condition of the procedure with identifier $k_i\in\text{FuncID}$.
With the function hypothesis, \textsc{hoare-call} can determine the effect of procedure call by looking up the callee's specification in $\Delta$.

Shallow embeddings of judgements involving procedure calls\cite{o2004separation} are different from those in section~\ref{sec:embed}.
Taking the denotational semantics based shallow embedding $\vDash_b$ for example, we introduce $\eta$ in \eqref{eq:eta}, a mapping from procedures $k_i$ to their denotations, to avoid circularity.
\begin{equation}
    \eta\in \text{FuncID} \rightarrow \text{state} \rightarrow \text{state} \rightarrow \text{exit\_kind} \rightarrow \text{Prop}
\label{eq:eta}    
\end{equation}
We use $\eta(k_i)$ to lookup procedure's denotation and $c\doublebrackets{\eta}$ to represent the program after substituting call to procedures by their denotations.
The shallow embedding $\triple{P_i}{k_i}{Q_i}_{\text{for } i \leq n} \vDash_b \triple{P}{c}{Q, [\vec{R}]}$ 
is defined as:\linebreak
for any $\eta$, $\vDash_b \triple{P_i}{\eta(k_i)}{Q_i, [\bot, \bot]}$ for all $i \leq n$ can imply $\vDash_b \triple{P}{c\doublebrackets{\eta}}{Q, [\vec{R}]}$.
% The rule \textsc{hypo-frame} can be proved for this shallow embedding\cite{}

% Deeply embedded Hoare logic using the judgement with function hypothesis needs a different validity definition and a different soundness theorem \cite{apt2010verification} from those in section~\ref{sec:embed}.
% % TODO: deep embed 下 hypo-frame 的证明？
% % FIXME: 以denotational semantics为例
% The main idea is to define a hypothetical validity.
% Taking the denotational semantics based validity $\vDash_b$ for example, let $\eta$ be a mapping from procedures $k_i$ to their denotations.
% To avoid circularity, we use $\eta(k_i)$ to lookup procedure's denotation and $c\doublebrackets{\eta}$ to represent the program after substituting call to procedures by their denotations.
% We define $\triple{P_i}{k_i}{Q_i}_{\text{for } i \leq n} \vDash_b \triple{P}{c}{Q, [\vec{R}]}$ iff. 
% $\vDash_b \triple{P_i}{\eta(k_i)}{Q_i, [\bot, \bot]}$ for all $i \leq n$ can imply $\vDash_b \triple{P}{c\doublebrackets{\eta}}{Q, [\vec{R}]}$.

% Specifically, for a given validity definition $\vDash_x$ in section~\ref{sec:embed}, we define}
% % For some shallow embedding $\vDash_x$, this judgement is defined based on the original Hoare triple embedding in section~\ref{sec:embed}: 
% \linebreak$\triple{P_i}{k_i}{Q_i}_{\text{for } i \leq n} \vDash_x \triple{P}{c}{Q, [\vec{R}]}$ iff. $\vDash_x \triple{P_i}{k_i}{Q_i, [\bot, \bot]}$ for all $i \leq n$ can imply $\vDash_x \triple{P}{c}{Q, [\vec{R}]}$.

\begin{figure}[h]
\paragraph{While-CF with Memory Operations and Procedure Calls}
$$
\begin{array}{rcl}
c \in \text{command} &:=& \cdots \ \mid \ x = [y] \ \mid \ [x] = y \ \mid \ \text{call} \ f()
\end{array}
$$
\paragraph{Procedure Call Proof Rules}
\begin{mathpar}
    % \inferrule[hoare-load]{}{
    %     \vdash \triple{l \mapsto v \land \doublebrackets{y} = l}{\ \ x = [y] \ \ }{l \mapsto v \land  \doublebrackets{x} = v \land \doublebrackets{y} = l, [\bot, \bot]}}
    % \and
    % \inferrule[hoare-store]{}{
    %     \vdash \triple{l \mapsto v \land \doublebrackets{x} = l \land \doublebrackets{y} = u}{\ \ [x] = y \ \ }{l \mapsto u \land \doublebrackets{x} = l \land \doublebrackets{y} = u, [\bot, \bot]}}
    % \and
    % \inferrule[frame]{
    %     c \text{ does not modify program variables freely occur } $F$ \\\\
    %     \vdash \triple{P}{c}{Q, [Q_{\text{brk}}, Q_{\text{con}}]}
    % }{
    %     \vdash \triple{P * F}{c}{Q * F, [Q_{\text{brk}} * F, Q_{\text{con}} * F]}
    % }
    % \and
    \inferrule[hoare-call]{}{
        \triple{P_i}{k_i}{Q_i}_{\text{for } i \leq n} \vdash \triple{P_i}{ \ \ \text{call} \ k_i \ \ }{Q_i, [\bot, \bot]}
    }
    \and
    \inferrule[hypo-frame]{
        c \text{ modifies program variables freely occuring in } R \text{ only through } k_i \\\\
        \triple{P_i}{k_i}{Q_i}_{\text{for } i \leq n} \vdash \triple{P}{c}{Q, [Q_{\text{brk}}, Q_{\text{con}}]}
    }{
        \triple{P_i*R}{k_i}{Q_i*R}_{\text{for } i \leq n} \vdash \triple{P*R}{c}{Q*R,  [Q_{\text{brk}} * R, Q_{\text{con}} * R]}
    }
\end{mathpar}
    \caption{Additional Proof Rules for Separation Logics and Procedure Calls}
    \label{fig:sep-call}
\end{figure}

In a logic combining separation logic and procedure call, we can generalize the \textsc{frame} rule to the \textsc{hypothetical-frame} rule in figure~\ref{fig:sep-call}, which was first proposed by O'Hearn \textit{et. al} \cite{o2004separation}.
This rule allows extend specifications of both the main program $c$ and procedures $k_i$ it invokes by composing an extra frame $R$ to their preconditions ($P_i$ and $P$) and postconditions ($Q_i$ and $Q$).
It is easily derivable in a deeply embedded logic by induction over the proof tree with modified atomic rules in section~\ref{sec:frame}, and it is proved for the shallow embedding we introduced in this section by O'Hearn \textit{et. al} \cite{o2004separation}.

% ex pre-/post-conditions of $k_i$'s function hypothesis.

%With these frame rules, we can better organize our proof by removing unnecessary assertion from the proof goal for simplification. 这句话我建议直接去掉，因为 remove 了能有任何好处吗？确实有，但是这里没说清楚。要说清楚的话，其实frame的作用是说：证明spec的时候可以只管local的有用的信息，而使用spec的时候可以用于不同的global的场景；而hypo-frame的作用则是可以在使用spec的时候忽略一些只与内部实现有关的separating conjunct

% Here, our judgement takes the form of $\Delta \vdash \triple{P}{c}{Q}$, where $\Delta$ is the function hypothesis (or type-context in VST), a list of function specifications $\triple{P_i}{k_i}{Q_i}$ for function identifiers $k_i$.
% Under the shallow embedding $\Delta \vDash \triple{P}{c}{Q}$ means, if every $\triple{P_i'}{k_i}{Q_i'}$ is valid then $\triple{P}{c}{Q}$ is valid.

% It is easily derivable in a deeply embedded logic by induction over the proof tree with modified atomic rules in section~\ref{sec:frame}, but it is invalid under shallow embeddings we have introduced.
% % Below gives an counterexample.
% In the counterexample below\footnote{The denotation of $k_1$ is trivial and $\eta$ is omitted in this example.}, we know $\vDash_b \triple{P_1}{k_1}{Q_1}$ is false (because location 0 is unavailable) and therefore $\vDash_b \triple{P_1}{k_1}{Q_1}$ implies everything including $\vDash_b \triple{P}{c}{Q}$.
% However, framing the pre/post-condition of $k_1$ with $R$, $\vDash_b \triple{P*R}{k_1}{Q*R}$ becomes true, but this does not imply $\vDash_b \triple{P*R}{c}{Q*R}$ to be true (location 1 is still unavailable).

% % $$
% \

% \begin{minipage}{\linewidth}
% \centering
% $k_1 \triangleq (x = [0])$ \ \
% $c \triangleq (x = [1])$ \ \
% $R \triangleq (0 \mapsto 1)$ \\
% $P_1 \triangleq Q_1 \triangleq \texttt{emp}$ \ \
% $P \triangleq Q \triangleq \texttt{emp}$
% % $\triple{P_1}{k_1}{Q_1}$ is false.\\
% % Therefore, $\triple{P_1}{k_1}{Q_1}$~implies~$\triple{P}{c}{Q}$.\\
% % And $\triple{P*R}{k_1}{Q*R}$ is true.\\
% % But $\triple{P*R}{c}{Q*R}$ is false.
% \end{minipage}

% \

% The reason for this rule to fail in the shallow embedding is that we do not know where function hypothesis are used for building the triple for the main program $c$.
% % O'Hearn \textit{et.} \cite{o2004separation} use a very special semantics to prove the \textsc{hypo-frame} rule and we believe its embedding is not general enough to fit into our evaluation.
% %这个说法也不好。这么说变成了我们的evaluation做的不充分。我觉得，应该直接说，
% In order to establish \textsc{hypo-frame} in a shallow embedding, it is inevitable to modify the definition of validity (like \cite{o2004separation}), which may break other formalized proofs.

% Notice that the counterexample does not invalidate \textsc{hypo-frame} in a deeply embedded logic.
% Because the premise $\triple{P_1}{k_1}{Q_1} \vdash \triple{P}{c}{Q}$ is not provable by any proof tree, even if it is valid under the shallow embedding.
% % TODO: remove this?
% This again reveals the fact that for a sound program logic, a provable judgement in the deep embedding implies its validity in some shallow embedding, but often not vice versa.


==> contents/fig/cont-embed-figure.tex <==
\begin{figure*}[ht]

\tikzstyle{progstate} = [circle, thick, minimum size = 0.5cm, text centered, draw = blue, fill=blue!10]
\tikzstyle{post} = [circle, thick, minimum size = 1cm, draw = orange, fill=orange!10]
\tikzstyle{guard} = [thick, draw = red, fill=red!10, fill opacity=0.5]
\tikzstyle{transition} = [->, draw=blue]
\centering

\begin{tikzpicture}[node distance = 1.5cm]

\draw[guard, dashed] (-0.9, -1.3) ellipse [x radius=1.5cm, y radius=0.8cm, rotate=10];
\draw[guard] (1.7, -1.5) ellipse [x radius=1.5cm, y radius=0.8cm, rotate=-20];
\draw[guard] (3.8, -0.2) ellipse [x radius=1.5cm, y radius=0.8cm, rotate=-15];
\draw[guard] (4.3, -1.3) ellipse [x radius=1.5cm, y radius=0.8cm, rotate=65];

\coordinate[label = right:\textcolor{red}{{$\guard{\cdot}{\ekc(\kappa_0)}$}}]() at (-3.6, -2.4);
\coordinate[label = right:\textcolor{red}{{$\guard{\cdot}{\ekc(\kappa)}$}}]() at (0.2, -2.7);
\coordinate[label = right:\textcolor{red}{{$\guard{\cdot}{\kappa}$}}]() at (0.8, 0.7);
\coordinate[label = right:\textcolor{red}{{$\guard{\cdot}{\ekb(\kappa)}$}}]() at (4.7, -2.2);

\node(P)[progstate] {\textcolor{blue}{$P$}};

\node(Qn)[post, below=1, right=70, label=right:\textcolor{orange}{$Q$}] at (P) {};
\node(Qr)[post, dashed, below=42, right=-44, label=left:\textcolor{orange}{$R_\ekc'$}] at (P) {};
\node(Qb)[post, below=52, right=37, label=right:\textcolor{orange}{$R_\ekc$}] at (P) {};
\node(Qc)[post, below=41, right=113, label=-100:\textcolor{orange}{$R_\ekb$}] at (P) {};

\node(Pn)[progstate, right=80] at (P) {};
% \node(Pc)[progstate, below=40, right=-40] at (P) {};
\node(Pb)[progstate, below=50, right=40] at (P) {};
\node(Pr)[progstate, below=40, right=120] at (P) {};

\draw[transition] (P) -- (Pn);
% \draw[transition] (P) -- (Pc);
\draw[transition] (P) -- (Pb);
\draw[transition] (P) -- (Pr);

% \draw[dashed, draw = red] (-0.9, -1.3) -- (1.7, -1.3);
\draw[dashed, thick, draw = red] (0.6, -1.3) -- (2.8, -1.3);
\draw[dashed, thick, draw = red] (-1, -2.1) -- (3.1, -2.1);
\draw[dashed, thick, draw = red] (-2.1, -1) -- (0.3, -1);

% \coordinate[label = right:\textcolor{blue}{$c/\ekr$}]() at (-0.7, -0.9);
\coordinate[label = right:\textcolor{blue}{$c/\ekc$}]() at (1, -1.1);
\coordinate[label = right:\textcolor{blue}{$c$}]() at (1.2, 0.2);
\coordinate[label = right:\textcolor{blue}{$c/\ekb$}]() at (1.5, -0.4);

\end{tikzpicture}


\caption{
    A Demo of Continuation based Shallow Embedding $\vDash_c \progspec{P}c\progspec{Q, [\vec{R}]}$}\label{fig:cont-embed}
\end{figure*}

==> contents/fig/figure_proof_destruct.tex <==
\begin{figure}[ht]
\tikzstyle{startstop} = [rectangle, minimum width = 1.5cm, minimum height = 0.5cm, text centered, draw = black]
\tikzstyle{arrow} = [thick, >= stealth]

\centering

\begin{tikzpicture}[node distance = 1.5cm]
\node(Tr0)[startstop] {\small \textcolor{blue}{$\triple{P}{c_1; c_2}{R}$}};
\node(Tr1)[startstop, above = 20] at (Tr0) {\small $\triple{P'}{c_1; c_2}{R'}$};
\node(Ent1L)[startstop, above = 10, left=50] at (Tr0) {\small $P \vdash P'$};
\node(Ent1R)[startstop, above = 10, right=50] at (Tr0) {\small $R' \vdash R$};
\node(Tr2)[startstop, above = 20] at (Tr1) {\small $\triple{P''}{c_1; c_2}{R''}$};
\node(Ent2L)[startstop, above = 10, left=50] at (Tr1) {\small $P' \vdash P''$};
\node(Ent2R)[startstop, above = 10, right=50] at (Tr1) {\small $R'' \vdash R'$};
\node(Tr3L)[startstop, above = 10, left=50] at (Tr2) {\small $\triple{P''}{c_1}{Q}$};
\node(Tr3R)[startstop, above = 10, right=50] at (Tr2) {\small $\triple{Q}{c_2}{R''}$};
\draw[arrow](Tr0) -- (Tr1);
\draw[arrow](Tr0) -- (Ent1L);
\draw[arrow](Tr0) -- (Ent1R);
\draw[arrow](Tr1) -- (Tr2);
\draw[arrow](Tr1) -- (Ent2L);
\draw[arrow](Tr1) -- (Ent2R);
\draw[arrow](Tr2) -- (Tr3L);
\draw[arrow](Tr2) -- (Tr3R);
\end{tikzpicture}

% TODO: larger arrow
\begin{tikzpicture}[node distance = 1.5cm]
\coordinate[label = right:{$\ \ \ \Downarrow \ \ \ $}](B) at(0, 0);
\coordinate[label = right:{$\ \ \ \Downarrow \ \ \ $}](B) at(1, 0);
\coordinate[label = right:{$\ \ \ \Downarrow \ \ \ $}](B) at(2, 0);
\end{tikzpicture}

\begin{tikzpicture}[node distance = 1.5cm]
\node(Tr0)[startstop] {\small \textcolor{blue}{$\triple{P}{c_1}{Q}$}};
\node(Tr1)[startstop, above = 20] at (Tr0) {\small $\triple{P'}{c_1}{Q}$};
\node(Ent1L)[startstop, above = 10, left=50] at (Tr0) {\small $P \vdash P'$};
\node(Tr2)[startstop, above = 30, left=1] at (Tr1) {\small $\triple{P''}{c_1}{Q}$};
\node(Ent2L)[startstop, above = 10, left=50] at (Tr1) {\small $P' \vdash P''$};
\draw[arrow](Tr0) -- (Tr1);
\draw[arrow](Tr0) -- (Ent1L);
\draw[arrow](Tr1) -- (Tr2);
\draw[arrow](Tr1) -- (Ent2L);
\end{tikzpicture}
~
\begin{tikzpicture}[node distance = 1.5cm]
\node(Tr0)[startstop] {\small \textcolor{blue}{$\triple{Q}{c_2}{R}$}};
\node(Tr1)[startstop, above = 20] at (Tr0) {\small $\triple{Q}{c_2}{R'}$};
\node(Ent1R)[startstop, above = 10, right=50] at (Tr0) {\small $R' \vdash R$};
\node(Tr2)[startstop, above = 30, right=1] at (Tr1) {\small $\triple{Q}{c_2}{R''}$};
\node(Ent2R)[startstop, above = 10, right=50] at (Tr1) {\small $R'' \vdash R'$};
\draw[arrow](Tr0) -- (Tr1);
\draw[arrow](Tr0) -- (Ent1R);
\draw[arrow](Tr1) -- (Tr2);
\draw[arrow](Tr1) -- (Ent2R);
\end{tikzpicture}
\caption{Destructing one proof tree and building new ones from its components}\label{fig:proof_tree_destruct}
\end{figure}

==> contents/fig/other_embed_table.tex <==
\begin{table}[h]
    \begin{center}
\resizebox{\textwidth}{!}{
    \begin{tabular}{ |c|c| } 
    \hline
        \begin{tabular}{c}
            \textbf{Verification Method}
        \end{tabular} & \begin{tabular}{c}
            \textbf{Corresponding Hoare Logic Embeddings}
        \end{tabular} \\
    \hline
    Hoare Monad \cite{nanevski2008hoare, nanevski2008ynot} & Shallow Embedding (BigS.) \\ \hline
    Dijkstra Monad \cite{swamy2013verifying, jacobs2015dijkstra, ahman2017dijkstra, maillard2019dijkstra} & Shallow Embedding (BigS.) \\ \hline
    CFML \cite{chargueraud2010program, chargueraud2011characteristic} & Deep Embedding \\ \hline
    \end{tabular}
}
    \end{center}
    \caption{Other verification methods and corresponding Hoare logic embeddings}
    \label{fig:table-other}
\end{table}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


